Solving the Two-dimensional single stock size Cutting Stock Problem with SAT and MaxSAT

Cutting rectangular items from stock sheets to satisfy demands while minimizing waste is a central manufacturing task. The Two-Dimensional Single Stock Size Cutting Stock Problem (2D-CSSP) generalizes bin packing by requiring multiple copies of each item type, which causes a strong combinatorial blow-up. We present a SAT-based framework where item types are expanded by demand, each copy has a sheet-assignment variable and non-overlap constraints are activated only for copies assigned to the same sheet. We also introduce an infeasible-orientation elimination rule that fixes rotation variables when only one orientation can fit the sheet. For minimizing the number of sheets, we compare three approaches: non-incremental SAT with binary search, incremental SAT with clause reuse across iterations and weighted partial MaxSAT. On the Cui--Zhao benchmark suite, our best SAT configurations certify two to three times more instances as provably optimal and achieve lower optimality gaps than OR-Tools, CPLEX and Gurobi. The relative ranking among SAT approaches depends on rotation: incremental SAT is strongest without rotation, while non-incremental SAT is more effective when rotation increases formula size.

==> Dih.tex <==
% Cac macro dau tieng Viet
\catcode`\@=11
\def\dd{\leavevmode\setbox0\hbox{d}\dimen@\wd0%
\rlap{\kern.3333\dimen@\raise1.2ex\vbox{\hrule width.5\dimen@}}d}

\def\DD{\leavevmode\setbox0\hbox{D}\dimen@\wd0%
\rlap{\kern.05\dimen@\raise0.8ex\vbox{\hrule width.5\dimen@}}D}

%\def\dd{d\kern-.46em\char '26}
%\def\DD{D\kern-.7em\raise0.4ex\hbox{\char '55}\kern.33em}
\def\is{\' \i }
\def\ih{\` \i }
\def\ihoi{\i \kern-.270em\raise.16ex\hbox{\char'47}\kern-.01em}
\def\inga{\~ \i }
\def\ing{\d i}
\def\ys{\' y}
\def\yh{\` y}
\def\yhoi{y\kern-.370em\raise.16ex\hbox{\char'47}\kern.1em}
\def\yn{\~ y}
\def\yng{\d y}
\def\as{\' a}
\def\ah{\` a}
\def\ahoi{a\kern-.370em\raise.16ex\hbox{\char'47}\kern.1em}
\def\an{\~ a}
\def\ang{\d a}
\def\us{\' u}
\def\uh{\` u}
\def\uhoi{u\kern-.370em\raise.16ex\hbox{\char'47}\kern.1em}
\def\un{\~ u}
\def\ung{\d u}
\def\es{\' e}
\def\eh{\` e}
\def\ehoi{e\kern-.370em\raise.16ex\hbox{\char'47}\kern.1em}
\def\en{\~ e}
\def\eng{\d e}
\def\os{\' o}
\def\oh{\` o}
\def\ohoi{o\kern-.370em\raise.16ex\hbox{\char'47}\kern.1em}
\def\on{\~ o}
\def\ong{\d o}
\def\oo{\^ o}
\def\oos{{\accent"5E o}\kern-.385em\raise.2ex
           \hbox{\char'23 }\kern-.1em}
\def\ooh{{\accent"5E o}\kern-.36em\raise.3ex
           \hbox{\char'22}\kern-.1em}
\def\oohoi{{\accent"5E o}\kern-.21em\raise.35ex
           \hbox{\char'47 }\kern-0.03em}
\def\oon{{\accent"5E o}\kern-.470em
           \raise.34ex\hbox{\char'176}}
\def\oong{\d {\accent"5E o}}
\def\aa{\^ a}
\def\aas{{\accent"5E a}\kern-.385em
       \raise.2ex\hbox{\char'23}\kern-.08em}
\def\aah{{\accent"5E a}\kern-.62em
       \raise.2ex\hbox{\char'22}\kern.12em}
\def\aahoi{{\accent"5E a}\kern-.21em
       \raise.35ex\hbox{\char'47 }\kern-.03em}
\def\aan{{\accent"5E a}\kern-.470em
       \raise.3ex\hbox{\char'176}}
\def\aang{\d {\accent"5E a}}
\def\ee{\^ e}
\def\ees{{\accent"5E e}\kern-.385em
       \raise.2ex\hbox{\char'23}\kern-.08em}
\def\eeh{{\accent"5E e}\kern-.62em
       \raise.2ex\hbox{\char'22}\kern.14em}
\def\eehoi{{\accent"5E e}\kern-.21em
       \raise.35ex\hbox{\char'47 }\kern-.01em}
\def\een{{\accent"5E e}\kern-.470em
       \raise.3ex\hbox{\char'176}}
\def\eeng{\d {\accent"5E e}}
\def\aw{\u a}
\def\aws{{\accent"15 a}\kern-.470em
       \raise.3ex\hbox{\char'23}\kern-.002em}
\def\awh{{\accent"15 a}\kern-.50em
       \raise.3ex\hbox{\char'22}\kern.05em}
\def\awhoi{{\accent"15 a}\kern-.410em
       \raise.3ex\hbox{\char'47}\kern.16em}
\def\awn{{\accent"15 a}\kern-.470em
       \raise.45ex\hbox{\char'176}}
\def\awng{\d {\accent"15 a}}
\def\uw{u\kern-.44em\raise.82ex\hbox{
       \vrule width .12em height .0ex depth .075ex 
       \kern-0.16em \char'56}\kern-.07em}
\def\uws{\' \uw }
\def\uwh{\` \uw }
\def\uwhoi{\uw \kern-.450em\raise.16ex
       \hbox{\char'47}\kern.175em}
\def\uwn{\~ \uw }
\def\uwng{\d \uw }
\def\ow{o\kern-.42em\raise.82ex\hbox{
       \vrule width .12em height .0ex depth .075ex 
       \kern-0.16em \char'56}\kern-.07em}
\def\ows{\' \ow }
\def\owh{\` \ow }
\def\owhoi{\ow \kern-.450em\raise.16ex
       \hbox{\char'47}\kern.175em}
\def\own{\~ \ow }
\def\owng{\d \ow }
\def\IS{\' I}
\def\IH{\` I}
\def\IHOI{I \kern-.63em\raise.80ex
       \hbox{\char'47}\kern.018em}
\def\INGA{\~ I}
\def\ING{\d I}
\def\YS{\' Y}
\def\YH{\` Y}
\def\YHOI{Y\kern-.46em\raise.80ex
       \hbox{\char'47}\kern.18em}
\def\YN{\~ Y}
\def\YNG{\d Y}
\def\AS{\' A}
\def\AH{\` A}
\def\AHOI{A\kern-.46em\raise.80ex\hbox{\char'47}\kern.18em}
\def\AN{\~ A}
\def\ANG{\d A}
\def\US{\' U}
\def\UH{\` U}
\def\UHOI{U\kern-.46em\raise.80ex\hbox{\char'47}\kern.18em}
\def\UN{\~ U}
\def\UNG{\d U}
\def\ES{\' E}
\def\EH{\` E}
\def\EHOI{E\kern-.46em\raise.80ex\hbox{\char'47}\kern.18em}
\def\EN{\~ E}
\def\ENG{\d E}
\def\OS{\' O}
\def\OH{\` O}
\def\OHOI{O\kern-.46em\raise.80ex\hbox{\char'47}\kern.2em}
\def\ON{\~ O}
\def\ONG{\d O}
\def\OO{\^ O}
\def\OOS{{\accent"5E O}\kern-.5em
      \raise.8ex\hbox{\char'23 }}
\def\OOH{{\accent"5E O}\kern-.48em
      \raise.9ex\hbox{\char'22}\kern-.08em}
\def\OOHOI{{\accent"5E O}\kern-.33em
      \raise1.02ex\hbox{\char'47 }\kern.04em}
\def\OON{{\accent"5E O}\kern-.60em
      \raise.9ex\hbox{\char'176}\kern.1em}
\def\OONG{\d {\accent"5E O}}
\def\AA{\^ A}
\def\AAS{{\accent"5E A}\kern-.5em
      \raise.8ex\hbox{\char'23 }}
\def\AAH{{\accent"5E A}\kern-.78em
      \raise.8ex\hbox{\char'22}\kern.28em}
\def\AAHOI{{\accent"5E A}\kern-.33em
      \raise1.02ex\hbox{\char'47 }\kern.04em}
\def\AAN{{\accent"5E A}\kern-.60em
      \raise.9ex\hbox{\char'176}\kern.07em}
\def\AANG{\d {\accent"5E A}}
\def\EE{\^ E}
\def\EES{{\accent"5E E}\kern-.5em
      \raise.8ex\hbox{\char'23 }}
\def\EEH{{\accent"5E E}\kern-.78em
      \raise.8ex\hbox{\char'22}\kern.28em }
\def\EEHOI{{\accent"5E E}\kern-.33em
      \raise1.02ex\hbox{\char'47 }\kern.04em}
\def\EEN{{\accent"5E E}\kern-.60em
      \raise.9ex\hbox{\char'176}\kern.1em}
\def\EENG{\d {\accent"5E E}}
\def\AW{\u A}
\def\AWS{{\accent"15 A}\kern-.620em
      \raise.85ex\hbox{\char'23}\kern.05em}
\def\AWH{{\accent"15 A}\kern-.60em
      \raise.85ex\hbox{\char'22}\kern.05em}
\def\AWHOI{{\accent"15 A}\kern-.530em
      \raise.88ex\hbox{\char'47}\kern.18em}
\def\AWN{{\accent"15 A}\kern-.57em
      \raise.97ex\hbox{\char'176}\kern.05em}
\def\AWNG{\d {\accent"15 A}}
\def\UW{U\kern-.42em\raise1.36ex\hbox{
      \vrule width .13em height .0ex depth .075ex 
      \kern-0.16em \char'56}\kern-.07em}
\def\UWS{\' \UW }
\def\UWH{\` \UW }
\def\UWHOI{\UW \kern-.48em\raise.80ex\hbox{\char'47}\kern.21em}
\def\UWN{\~ \UW }
\def\UWNG{\d \UW }
\def\OW{O\kern-.460em\raise1.36ex\hbox{
      \vrule width .13em height .0ex depth .075ex 
      \kern-0.16em \char'56}\kern-.07em}
\def\OWS{\' \OW }
\def\OWH{\` \OW }
\def\OWHOI{\OW \kern-.540em\raise.80ex\hbox{\char'47}\kern.25em}
\def\OWN{\~ \OW }
\def\OWNG{\d \OW }
\catcode`\@=\active

